Snowmass 2021 White Paper Instrumentation Frontier 05 -- White Paper 1: MPGDs: Recent advances and current R&D

This paper will review the origins, development, and examples of new versions of Micro-Pattern Gas Detectors. The goal for MPGD development was the creation of detectors that could cost-effectively cover large areas while offering excellent position and timing resolution, and the ability to operate at high incident particle rates. The early MPGD developments culminated in the formation of the RD51 collaboration which has become the critical organization for the promotion of MPGDs and all aspects of their production, characterization, simulation, and uses in an expanding array of experimental configurations. For the Snowmass 2021 study, a number of Letters of Interest were received that illustrate ongoing developments and expansion of the use of MPGDs. In this paper, we highlight high precision timing, high rate application, trigger capability expansion of the SRS readout system, and a structure designed for low ion backflow.

==> authorlist.tex <==
\Author{K.~Dehmelt$^{1,*,\dagger}$, A.~White$^{2,*,\dagger}$, %%%
M. Alviggi$^3$, M.T. Camerlingo$^4$, V. Canale$^3$, V. D'amico$^5$, M. Della Pietra$^{3,\dagger}$, C. Di Donato$^3$, R. Di Nardo$^5$, S. Franchellucci$^5$, P. Iengo$^6$, M. Iodice$^7$, F. Petrucci$^5$, G. Sekhniaidze$^8$, M. Sessa$^5$, %%%
Hans Muller$^{9, 18,\dagger}$, H.~Natal da Luz$^{10}$, S.~Popescu$^{11}$, L.~Scharenberg$^9$, K.~Gnanvo$^{12}$, A.~Rusu$^{13}$, D.~Pfeiffer$^{14, 15}$, R.~Hall-Wilton$^{15}$, J.~Toledo-Alarcon$^{16}$, M.~Lupberger$^9$, M.~Bregant$^{17}$, E.~Oliveri$^{18}$, %%%
Z.~Zhang$^{19,\dagger}$, J.~Liu$^{19}$, M.~Shao$^{19}$, Y.~Zhou$^{19}$, %%%
S.~Aune$^{20}$, D.~Desforge$^{20}$, I.~Giomataris$^{20}$, T.~Gustavsson$^{20}$, F.~J.~Iguaz1$^{3,4}$, M.~Kebbiri$^{20}$, P.~Legou$^{20}$, T.~Papaevangelou$^{20}$, M.~Pomorski$^{20}$, L.~Sohl$^{20}$, %%%
J.~Bortfeldt$^{18,22}$, F.~Brunbauer$^{18}$, K.~J.~Floethner$^{18}$, D.~Janssens$^{18}$, M.~Lisowska$^{18}$, M.~Lupberger$^{9,18}$, G.~Orlandini$^{18}$, F.~Resnati$^{18}$, L.~Ropelewski$^{18}$, L.~Scharenberg$^{18}$, T.~Schneider$^{18}$, M.~van Stenis$^{18}$, A.~Utrobicic$^{18}$, R.~Veenhof$^{18,23,24}$, S.~White$^{18,25,\dagger}$, %%%
Y.~Meng$^{19}$, X.~Wang$^{19}$, %%%
I.~Angelis$^{26}$, A.~Kallitsopoulou$^{26}$, K.~Kordas$^{26}$, C.~Lampoudis$^{26}$, I.~Maniatis$^{26}$, I.~Manthos$^{26,27}$, K.~Paraschou$^{26}$, D.~Sampsonidis$^{26}$, A.~Tsiamis$^{26}$, S.~E.~Tzamarias$^{26,\dagger}$, %%%
G.~Fanourakis$^{28}$, %%%
Y.~Tsipolitis$^{29}$, %%%
M.~Gallinaro$^{30}$, %%%
F.~Garcia$^{31}$, %%%
S.~Malace$^{12}$%%%
}
\noindent $^1$Stony Brook University, Stony Brook, NY, USA
\newline $^2$University of Texas, Arlington, TX, USA
\newline $^3$University and INFN Sez. Napoli, Naples, Italy
\newline $^4$University and INFN Sez. Roma Tre, Rome, Italy and CERN, Geneva, Switzerland
\newline $^5$University and INFN Sez. Roma Tre, Rome, Italy
\newline $^6$INFN Sez. Napoli, Naples, IT, and CERN, Geneva, Switzerland
\newline $^7$INFN Sez. Roma Tre, Rome, Italy
\newline $^8$INFN Sez. Napoli, Naples, Italy
\newline $^9$Bonn University, Bonn, Germany
\newline $^{10}$Czech Technical University Prague, Prague, Czech Republic
\newline $^{11}$Kansas University, USA
\newline $^{12}$JLab, Newport News, VA, USA
\newline $^{13}$SRS Technology, Meyrin, Switzerland
\newline $^{14}$Bicocca University, Milano, Italy
\newline $^{15}$ESS ERIC, Lund, Sweden
\newline $^{16}$Universitat Polit\`ecnica de Val\`encia, Val\`encia, Spain
\newline $^{17}$IFUSP, S\~ao Paulo, Brasil
\newline $^{18}$CERN, Geneva, Switzerland
\newline $^{19}$USTC, Hefei, China
\newline $^{20}$CEA Saclay, France
\newline $^{21}$Synchrotron Soleil, Gif-sur-Yvette, France
\newline $^{22}$LMU Munich, Germany
\newline $^{23}$MEPhI Moscow, Russian Federation
\newline $^{24}$Uludag University, Turkey
\newline $^{25}$University of Virginia, Charlottesville, VA, USA
\newline $^{26}$Aristotle University of Thessaloniki, Greece
\newline $^{27}$University of Birmingham, UK
\newline $^{28}$NCSR Demokritos, Athens, Greece
\newline $^{29}$National Technical University of Athens, Greece
\newline $^{30}$LIP Lisboa, Portugal
\newline $^{31}$Helsinki Institute of Physics, Helsinki, Finland

\noindent$^*$ White Paper Coordinators
\newline\noindent$\dagger$ Corresponding LOI author

